Averages of b-hadron and c-hadron Properties at the End of 2007

This article reports world averages for measurements of b-hadron and c-hadron properties obtained by the Heavy Flavor Averaging Group (HFAG) using the results available at the end of 2007. For the averaging, common input parameters used in the various analyses are adjusted (rescaled) to common values, and known correlations are taken into account. The averages include branching fractions, lifetimes, neutral meson mixing parameters, CP violation parameters, and parameters of semileptonic decays.

==> b2charm_end_of_2007_v001.tex <==
\input{b2charm_end_of_2007_v001_preamble.tex} 
\input{b2charm_end_of_2007_v001_symbols.tex} 

\begin{document} 
\input{b2charm_end_of_2007_v001_blurb.tex} 
\clearpage 
\input{b2charm_end_of_2007_v001_tables.tex} 
\end{document} 




==> charm/charm_bibliography.tex <==
%----section 1 (Alan) --------------------------------------------------

\bibitem{belle_kk} M. Staric {\it et al.} (Belle Collab.),
                Phys. Rev. Lett. {\bf 98}, 211803 (2007).

\bibitem{babar_kpi} B. Aubert {\it et al.} (BaBar Collab.), 
                Phys. Rev. Lett. {\bf 98}, 211802 (2007).

\bibitem{cdf_kpi} T. Aaltonen {\it et al.} (CDF Collab.), 
                Phys. Rev. Lett. {\bf 100}, 121802 (2008).

\bibitem{hfag_charm} http://www.slac.stanford.edu/xorg/hfag/charm/index.html

\bibitem{BigiUraltsev} I. Bigi and N. Uraltsev,
                 Nucl. Phys.~B {\bf 592}, 92 (2001).

\bibitem{Petrov} For a survey of predictions see:
           A.~A. Petrov, eConf {\bf C030603} (2003), arXiv:hep-ph/0311371; 
           Nucl. Phys. Proc. Suppl. {\bf 142}, 333 (2005).

\bibitem{Falk} A.~F. Falk {\it et al.},
%Y.\ Grossman, Z.\ Ligeti, Y.\ Nir, and A.\,A.\,Petrov, 
Phys. Rev.~D {\bf 69}, 114021 (2004).

\bibitem{semi_references}
E.~M. Aitala {\it et al.} (E791 Collab.),
           Phys. Rev. Lett. {\bf 77}, 2384 (1996);

C. Cawlfield {\it et al.} (CLEO Collab.),
           Phys. Rev.~D {\bf 71}, 071101 (2005);

B. Aubert {\it et al.} (BaBar Collab.),
           Phys. Rev.~D {\bf 76}, 014018 (2007);

U. Bitenc {\it et al.} (Belle Collab.),
           Phys. Rev.~D {\bf 77}, 112003 (2008).

\bibitem{ycp_fnal}
E.~M. Aitala {\it et al.} (E791 Collab.),
           Phys. Rev. Lett. {\bf 83}, 32 (1999);

J.~M. Link {\it et al.} (FOCUS Collab.),
           Phys. Lett.~B {\bf 485}, 62 (2000);

\bibitem{ycp_cleo}
S.~E. Csorna {\it et al.} (CLEO Collab.),
           Phys. Rev.~D {\bf 65}, 092001 (2002);

\bibitem{ycp_babar}
B. Aubert {\it et al.} (BaBar Collab.), arXiv:0712.2249
           (submitted to Phys. Rev.~D).

\bibitem{kspp_references} 
D.~M. Asner {\it et al.} (CLEO Collab.),
           Phys. Rev.~D {\bf 72}, 012001 (2005);
	   arXiv:hep-ex/0503045 (revised April 2007);

L.~M. Zhang {\it et al.} (Belle Collab.),
           Phys. Rev. Lett. {\bf 99}, 131803 (2007).

\bibitem{belle_kpi} 
L.~M. Zhang {\it et al.} (Belle Collab.),
           Phys. Rev. Lett. {\bf 96}, 151801 (2006).

\bibitem{knpi_references}
W. Lockman (Belle Collab.), presented at LP'07, Daegu, S. Korea 
(13 August 2007);

See also: X.~C. Tian {\it et al.} (Belle Collab.),
           Phys. Rev. Lett. {\bf 95}, 231801 (2005).

\bibitem{cleoc}
D.~M. Asner {\it et al.} (CLEOc Collab.), arXiv:0802.2268
           (submitted to Phys. Rev.~D).

\bibitem{MINUIT} See\,\ 
{\tt http://wwwasdoc.web.cern.ch/wwwasdoc/minuit/minmain.html}


%----section 2 (Bostjan)--------------------------------------------------

\bibitem{pdg} W.-M. Yao {\it et al.} (Particle Data Group),
  J. Phys.~G {\bf 33}, 1 (2006).

\bibitem{babar1} B. Aubert {\it et al.} (BaBar Collab.),
  Phys. Rev. Lett. {\bf 90}, 242001 (2003).

\bibitem{cleo1} D. Besson {\it et al.} (CLEO Collab.),
   Phys. Rev.~D {\bf 68}, 032002 (2003).

\bibitem{belle1} K. Abe {\it et al.} (Belle Collab.), 
Phys. Rev.~D {\bf 69}, 112002 (2004). 

 \bibitem{focus1} J.~M. Link {\it et al.} (Focus Collab.),
  Phys. Lett.~B {\bf 586}, 11 (2004).

\bibitem{theory1} S. Godfrey, N. Isgur, Phys. Rev.~D {\bf 32}, 189 (1985); 
  J.~L. Rosner, Comm. Nucl. Part. Phys. {\bf 16}, 109 (1986); 
  S. Godfrey, R. Kokoski, Phys. Rev.~D {\bf 43}, 1679 (1991); 
  N. Isgur, B. Wise, Phys. Rev. Lett. {\bf 66}, 1130 (1991); 
  M. Di Pierro, E. Eichten, Phys. Rev.~D {\bf 64}, 114004 (2001). 

 \bibitem{theory2} P. Colangelo, F. De Fazio, R. Ferrandes,
   Mod. Phys. Lett.~A {\bf 19}, 2083 (2004); 
   F. Jugeau {\it et al.}, Phys. Rev.~D {\bf 72}, 094010 (2005).

\bibitem{theory3}  
  R.~N. Cahn, J.~D. Jackson, Phys. Rev.~D {\bf 68}, 037502 (2003).

\bibitem{theory4} T. Barnes, F.~E. Close, H.~J. Lipkin,  
   Phys. Rev.~D {\bf 68}, 054065 (2003); 
   H.~J. Lipkin, Phys. Lett.~B {\bf 580}, 50 (2004).

\bibitem{theory5} W.~A. Bardeen, E.~J. Eichten, C.~T. Hill,  
   Phys. Rev.~D {\bf 68}, 054024 (2003).


\bibitem{belle2} A. Kuzmin {\it et al.} (Belle Collab.),
  Phys. Rev.~D {\bf 76}, 012006 (2007).

 \bibitem{cdf1} A. Abulencia {\it et al.} (CDF Collab.),
  Phys. Rev.~D {\bf 73}, 051104 (2006).

\bibitem{belle3} K. Abe {\it et al.} (Belle Collab.),
  Phys. Rev. Lett. {\bf 94}, 221805 (2005).

% D_s**
\bibitem{belle4} Y. Mikami {\it et al.} (Belle Collab.),
  Phys. Rev. Lett. {\bf 92}, 012002 (2004).

\bibitem{babar4} B. Aubert {\it et al.} (BaBar Collab.), 
   Phys. Rev.~D {\bf 74}, 032007 (2006).

\bibitem{belle8} J. Brodzicka {\it et al.} (Belle Collab.),
   Phys. Rev. Lett. {\bf 100}, 092001 (2008).

\bibitem{babar3} B. Aubert {\it et al.} (BaBar Collab.),
  Phys. Rev. Lett. {\bf 97}, 222001 (2006).

\bibitem{selex1} A.~V. Evdkimov {\it et al.} (Selex Collab.),
  Phys. Rev. Lett. {\bf 93}, 242001 (2004).

\bibitem{belle5} P. Krokovny {\it et al.} (Belle Collab.),
  Phys. Rev. Lett. {\bf 91}, 262002 (2003).

\bibitem{babar6} B. Aubert {\it et al.} (BaBar Collab.),
  Phys. Rev. Lett. {\bf 93}, 181801 (2004).

\bibitem{belle6} A. Drutskoy {\it et al.} (Belle Collab.),
  Phys. Rev. Lett. {\bf 94}, 061802 (2005).

\bibitem{belle7} V. Balagura {\it et al.} (Belle Collab.),
  Phys. Rev.~D {\bf 77}, 032001 (2008).

\bibitem{babar2} B. Aubert {\it et al.} (BaBar Collab.), 
  Phys. Rev.~D {\bf 77}, 011102(R) (2008). 

\bibitem{aleph1} A. Heister {\it et al.} (ALEPH Collab.),
  Phys. Lett.~B {\bf 526}, 34 (2002).

\bibitem{babar5} B. Aubert {\it et al.} (BaBar Collab.), 
  Phys. Rev.~D {\bf 74}, 031103(R) (2006).

%----section 3 (Milind)--------------------------------------------------

\bibitem{Becher:2005bg}
T.~Becher and R.~J. Hill, Phys. Lett.~B {\bf 633}, 61 (2006).

\bibitem{Kobayashi:1973fv}
M.~Kobayashi and T.~Maskawa, Prog. Theor. Phys. {\bf 49}, 652 (1973).

\bibitem{Gilman:1989uy}
F.~J. Gilman and R.~L. Singleton, Phys. Rev.~D {\bf 41}, 142 (1990).

\bibitem{Boyd:1994tt}
C.~G. Boyd, B.~Grinstein, and R.~F. Lebed, Phys. Rev. Lett. {\bf 74},
  4603 (1995).

\bibitem{Hill:2006ub} R.~J. Hill, arXiv:hep-ph/0606023 (2006).

\bibitem{Becirevic:1999kt}
D.~Becirevic and A.~B. Kaidalov, Phys. Lett.~B {\bf 478}, 417 (2000).

\bibitem{Huang:2004fra}
G.~S. Huang {\em et~al.}, Phys. Rev. Lett. {\bf 94}, 011802 (2005).

\bibitem{Link:2004dh}
J.~M. Link {\em et~al.}, Phys. Lett.~B {\bf 607}, 233 (2005).

\bibitem{Widhalm:2006wz}
L.~Widhalm {\em et~al.}, Phys. Rev. Lett. {\bf 97}, 061804 (2006).

\bibitem{Aubert:2006mc}
B.~Aubert {\em et~al.}, Phys. Rev.~D {\bf 76}, 052005 (2007).

\bibitem{GaoICHEP06}
Y.~Gao, Talk presented at the XXXIII International Conference on High Energy
  Physics (ICHEP'06), Moscow, the Russian Federation, August 2006.

%\bibitem{CroninHennessy:2007se}
%D.~Cronin-Hennessy {\em et~al.}, arXiv:0712.0998 (2007).

\bibitem{Dobbs:2007sm}
S. Dobbs {\em et~al.}, arXiv:0712.1020 (2007).

\bibitem{Aubin:2004ej}
C.~Aubin {\em et~al.}, Phys. Rev. Lett. {\bf 94}, 011601 (2005).

\bibitem{Boyd:1997qw}
C.~G. Boyd and M.~J. Savage, Phys. Rev.~D {\bf 56}, 303 (1997).

\bibitem{Arnesen:2005ez}
M.~C. Arnesen, B.~Grinstein, I.~Z. Rothstein, and I.~W. Stewart, 
 Phys. Rev. Lett. {\bf 95}, 071802 (2005).

\bibitem{Bourrely:1980gp}
C.~Bourrely, B.~Machet, and E.~de~Rafael, 
Nucl. Phys.~B {\bf 189}, 157 (1981).

%\bibitem{Ball:2006yd}
%P.~Ball, Phys. Lett., {\bf B641}, pp.~50--56, 2006.

\bibitem{E691:90}
J.~C. Anjos {\em et~al.}, Phys. Rev. Lett. {\bf 65}, 2630 (1990).

\bibitem{E653:92}
K.~Kodama {\em et~al.}, Phys. Lett.~B {\bf 274}, 246 (1992).

\bibitem{E687:93}
P.~L. Frabetti {\em et~al.}, Phys. Lett.~B {\bf 307}, 262 (1993).

\bibitem{E791:98a}
E.~M. Aitala {\em et~al.}, Phys. Rev. Lett. {\bf 80}, 1393 (1998).

\bibitem{E791:98b}
E.~M. Aitala {\em et~al.}, Phys. Lett.~B {\bf 440}, 435 (1998).

\bibitem{BEATRICE:99}
M.~Adamovich {\em et~al.}, Eur. Phys. J.~C {\bf 6}, 35 (1999).

\bibitem{FOCUS:02b}
J.~M. Link {\em et~al.}, Phys. Lett.~B {\bf 544}, 89 (2002).

\bibitem{FOCUS:05}
J.~M. Link {\em et~al.}, Phys. Lett.~B {\bf 607}, 67 (2005).

\bibitem{BaBar:06} B.~Aubert {\em et~al.}, arXiv:hep-ex/0607085 (2006).

\bibitem{Mahlke07} H.~Mahlke, arXiv:hep-ex/0702014 (2007).

\bibitem{FOCUS:02a}
J.~M. Link {\em et~al.}, Phys. Lett.~B {\bf 535}, 43 (2002).

\bibitem{Wiss07} J.~Wiss, arXiv:0709.3247 (2007).

%----section 4 (Daniel CP)--------------------------------------------

\bibitem{BigiSanda} I.~I. Bigi and A.~I. Sanda, 
{\em CP Violation\/}, Cambridge University Press (2000).

\bibitem{Nir} Y. Nir, arXiv:hep-ph/9911321 (1999).

\bibitem{Buccella} F. Buccella {\it et al.}, 
Phys. Rev.~D {\bf 51}, 3478 (1995).
 
\bibitem{BaBar2008} B. Aubert {\it et al.} (BaBar Collab.), 
Phys. Rev. Lett. {\bf 100}, 061803 (2008).

\bibitem{CDF2005} D. Acosta {\it et al.} (CDF Collab.), 
Phys. Rev. Lett. {\bf 94}, 122001 (2005).

\bibitem{FOCUS2000} J.~M. Link {\it et al.} (FOCUS Collab.), 
Phys. Lett.~B {\bf 491}, 232 (2000); 
Err., Phys. Lett.~B {\bf 495}, 443 (2000).

\bibitem{E7911998} E.~M. Aitala {\it et al.} (E791 Collab.), 
Phys. Lett.~B {\bf 421}, 405 (1998).

\bibitem{CLEO1995} J.~E. Bartelt {\it et al.} (CLEO Collab.), 
Phys. Rev.~D {\bf 52}, 4860 (1995).

\bibitem{E6871994} P.~L. Frabetti {\it et al.} (E687 Collab.), 
Phys. Rev.~D {\bf 50}, 2953 (1994).

\bibitem{CLEO2001} G. Bonvicini {\it et al.} (CLEO Collab.), 
Phys. Rev.~D {\bf 63}, 071101 (2001).
 
\bibitem{BaBar2008b} B. Aubert {\it et al.} (BaBar Collab.), 
arXiv:0802.4035 (2008).

\bibitem{Belle2008} K. Arinstein {\it et al.} (Belle Collab.), 
Phys. Lett.~B {\bf 662}, 102 (2008).

\bibitem{CLEO2005} D. Cronin-Hennessy {\it et al.} (CLEO Collab.), 
Phys. Rev.~D {\bf 72}, 031102 (2005).

\bibitem{CLEOc2007} S. Dobbs {\it et al.} (CLEOc Collab.), 
Phys. Rev.~D {\bf 76}, 112001 (2007). 

\bibitem{CLEO2001a} S. Kopp {\it et al.} (CLEO Collab.), 
Phys. Rev.~D {\bf 63}, 092001 (2001).

\bibitem{Belle2005} X.~C. Tian {\it et al.} (Belle Collab.), 
Phys. Rev. Lett. {\bf 95}, 231801 (2005).

\bibitem{CLEO2001b} G. Brandenburg {\it et al.} (CLEO Collab.), 
Phys. Rev. Lett. {\bf 87}, 071802 (2001).

\bibitem{CLEO2004} D.~M. Asner {\it et al.} (CLEO Collab.), 
Phys. Rev.~D {\bf 70}, 091101 (2004).

\bibitem{FOCUS2005} J.~M. Link {\it et al.} (FOCUS Collab.), 
Phys. Lett.~B {\bf 622}, 239 (2005).

\bibitem{FOCUS2002} J.~M. Link {\it et al.} (FOCUS Collab.), 
Phys. Rev. Lett. {\bf 88}, 041602 (2002); 
Err., Phys. Rev. Lett. {\bf 88}, 159903 (2002).

\bibitem{E7911997} E.~M. Aitala {\it et al.} (E791 Collab.), 
Phys. Lett.~B {\bf 403}, 377 (1997).

\bibitem{BaBar2005} B. Aubert {\it et al.} (BaBar Collab.), 
Phys. Rev.~D {\bf 71}, 091101 (2005).


%----section 5 (Daniel T)--------------------------------------------

\bibitem{Valencia} E.~Golowich and G.~Valencia, 
Phys. Rev.~D {\bf 40}, 112 (1989).

\bibitem{Bigi} I.~I. Bigi, in Proceedings of KAON2001: 
Inter. Conf. on \cp\ Violation, Pisa, Italy, 12-17 Jun 2001, p.417 
(arXiv:hep-ph/0107102).

\bibitem{Bensalem} W.~Bensalem, A.~Datta and D.~London, 
Phys. Rev.~D {\bf 66}, 094004 (2002);
W. Bensalem and D. London, Phys. Rev.~D {\bf 64}, 116003 (2001).

\bibitem{Bensalem2} W.~Bensalem, A.~Datta and D.~London, 
Phys. Lett.~B {\bf 538}, 309 (2002).




==> slbdecays/README <==
	README  (Last update: 28 April 12, Francesca Di Lodovico)

- This directory (Papers/EndOfYear07/slbdecays) 
contains all the tex files for the semileptonic averages.
They are:

	mail file: slbdecays.tex
	common params: common.tex
	exclusive b->clnu: exclusiveclnu.tex
	inclusive b->lcnu: inclusiveclnu.tex
	exclusive b->clnu: exclusiveulnu.tex
	inclusive b->lcnu: inclusiveulnu.tex
	references: slb_refs.tex
	appendix: slb_app.tex	

- The tables are in:
	EndOfYear07/tables/slb


- The figures are in:
	EndOfYear07/figures/slb


- Just for testing the semileptonic text un-comment:
	\input{slbdecays/slbdecays.tex} 
	\input{slbdecays/slb_app.tex}
	\input{hfag_ref}

from EndOfYear07/EndOfYear07.tex

- to run latex, go in the directory EndOfYear07 and run:

	make clean; latex  EndOfYear07.tex; latex  EndOfYear07.tex; make default

The EndOfYear07.ps file will be produced.




==> slbdecays/slb_app.tex <==
\section{Methodology}
\label{sec:slmethodology}
The general method used in HFAG for extracting averages is described in our previous
update~\cite{hfag_hepex_endof2006}.
In the following, the method has been
extended to take into account the fact that measurement errors often
depend on the measured value, i.e. are relative errors.
Furthermore, an effort has been made to separate statistical, and
different sources of systematic and theoretical errors.

For measurements with Gaussian errors, the usual estimator for the
average of a set of measurements is obtained by minimizing the following
$\chi^2$:
\begin{equation}
\chi^2(t) = \sum_i^N \frac{\left(y_i-t\right)^2}{\sigma^2_i} ,
\label{eq:chi2t}
\end{equation}
where $y_i$ is the measured value for input $i$ and $\sigma_i^2$ is the
variance of the distribution from which $y_i$ was drawn.  The value $\hat{t}$
of $t$ at minimum $\chi^2$ is our estimator for the average.  (This
discussion is given for independent measurements for the sake of
simplicity; the generalization to correlated measurements is
straightforward, and has been used when averaging results.) 
The true $\sigma_i$ are unknown but typically the error as assigned by the
experiment $\sigma_i^{\mathrm{raw}}$ is used as an estimator for it.
Caution is advised,
however, in the case where $\sigma_i^{\mathrm{raw}}$
depends on the value measured for $y_i$. Examples of this include
an uncertainty in any multiplicative factor (like
an acceptance) that enters the determination of $y_i$, i.e. the $\sqrt{N}$
dependence of Poisson statistics, where $y_i \propto N$
and $\sigma_i \propto \sqrt{N}$.
Failing to account for this type of
dependence when averaging leads to a biased average.
Biases in the average can be avoided (or at least reduced)
by minimizing the following
$\chi^2$:
\begin{equation}
\chi^2(t) = \sum_i^N \frac{\left(y_i-t\right)^2}{\sigma^2_i(\hat{t})} .
\label{eq:chi2that}
\end{equation}
In the above $\sigma_i(\hat{t})$ is the uncertainty
assigned to input $i$ that includes the assumed dependence of the
stated error on the value measured.  As an example, consider 
a pure acceptance error, for which
$\sigma_i(\hat{t}) = (\hat{t} / y_i)\times\sigma_i^{\mathrm{raw}}$ .
It is easily verified that solving Eq.~\ref{eq:chi2that} 
leads to the correct behavior, namely
$$ 
\hat{t} = \frac{\sum_i^N y_i^3/(\sigma_i^{\mathrm{raw}})^2}{\sum_i^N y_i^2/(\sigma_i^{\mathrm{raw}})^2},
$$
i.e. weighting by the inverse square of the 
fractional uncertainty, $\sigma_i^{\mathrm{raw}}/y_i$.

It is sometimes difficult to assess the dependence of $\sigma_i^{\mathrm{raw}}$ on
$\hat{t}$ from the errors quoted by experiments.  
%An example is the
%uncertainty on a branching fraction, $\mathcal{B}=(N-B)/\eff$, due to
%a change in the background modeling.   
%As a result, the sensitivity
%to different assumptions on these dependences has been
%studied for the averages given in this section.

Another issue that needs careful treatment is the question of correlation
among different measurements, e.g. due to using the same theory for
calculating acceptances.  A common practice is to set the correlation
coefficient to unity to indicate full correlation.  However, this is
not a ``conservative'' thing to do, and can in fact lead to a significantly
underestimated uncertainty on the average.  In the absence of
better information, the most conservative choice of correlation coefficient
between two measurements $i$ and $j$
is the one that maximizes the uncertainty on $\hat{t}$
due to that pair of measurements:
\begin{equation}
\sigma_{\hat{t}(i,j)}^2 = \frac{\sigma_i^2\,\sigma_j^2\,(1-\rho_{ij}^2)}
   {\sigma_i^2 + \sigma_j^2 - 2\,\rho_{ij}\,\sigma_i\,\sigma_j} ,
\label{eq:correlij}
\end{equation}
namely
\begin{equation}
\rho_{ij} = \mathrm{min}\left(\frac{\sigma_i}{\sigma_j},\frac{\sigma_j}{\sigma_i}\right) ,
\label{eq:correlrho}
\end{equation}
which corresponds to setting $\sigma_{\hat{t}(i,j)}^2=\mathrm{min}(\sigma_i^2,\sigma_j^2)$.
Setting $\rho_{ij}=1$ when $\sigma_i\ne\sigma_j$ can lead to a significant
underestimate of the uncertainty on $\hat{t}$, as can be seen
from Eq.~\ref{eq:correlij}.

Finally, a note on the breakdown of the error sources
contributing to the overall uncertainty on the average.
The overall covariance matrix is constructed from a number of
individual sources, e.g.
$\mathbf{V} = \mathbf{V_{stat}+V_{sys}+V_{th}}$.
The variance on the average $\hat{t}$ can be written
\begin{eqnarray}
\sigma^2_{\hat{t}} 
 &=& 
\frac{ \sum_{i,j}\left(\mathbf{V^{-1}}\, 
\mathbf{[V_{stat}+V_{sys}+V_{th}]}\, \mathbf{V^{-1}}\right)_{ij}}
{\left(\sum_{i,j} V^{-1}_{ij}\right)^2}
= \sigma^2_{stat} + \sigma^2_{sys} + \sigma^2_{th} .
\end{eqnarray}
Written in this form, one can readily determine the 
contribution of each source of uncertainty to the overall uncertainty
on the average.  This breakdown of the uncertainties is used below.



==> tables/slb/BLL.tex <==

\begin{table}[!htb]
\caption{Summary of inclusive determinations of $\vub$ in the BLL prescription.
  The errors quoted on \vub\ correspond to
experimental and theoretical uncertainties, respectively. }
\begin{center}
\begin{small}
\begin{tabular}{|llcc|}
\hline
& accepted region & $f_u$
&  $\Vub [10^{-3}]$\\
\hline\hline
BELLE~\cite{ref:belle-mxq2Anneal}
& $M_X<1.7\,\gev/c^2, q^2>8\,\gev^2/c^2$ & 0.26
& $4.72 \pm 0.50 \pm 0.35$ \\ 
\babar~\cite{ref:babar-q2mx}
& $M_X<1.7\,\gev/c^2, q^2>8\,\gev^2/c^2$ & 0.26
& $5.12 \pm 0.38 \pm 0.38$ \\ 
BELLE~\cite{ref:belle-mx}
& $M_X<1.7\,\gev/c^2, q^2>8\,\gev^2/c^2$ & 0.26
& $5.04 \pm 0.39 \pm 0.37$ \\ 
\hline\hline
{\bf Average}
& \mathversion{bold}$\chi^2=0.5/2$, \mathversion{bold} CL$=0.77$ &
& \mathversion{bold}$5.02 \pm 0.26 \pm 0.37$ \\
\hline
\end{tabular}\\
\end{small}
\end{center}
\label{tab:bulnuBLL}
\end{table}

\begin{table}[!htb]
\caption{Summary of uncertainties on $\vub$ in the BLL prescription.}
\begin{center}
\begin{small}
\begin{tabular}{|lr|} \hline
  Source & Uncertainty(\%) \\ \hline\hline
  Statistics & $\pm3.2$ \\
  Detector & $\pm2.9$ \\
  $B\to X_c l \nu$ model & $\pm1.8$ \\
  $B\to X_u l \nu$ model & $\pm2.4$ \\
  Spectral fraction ($m_b$) & $\pm3.0$ \\
  Perturbative : Strong coupling $\alpha_s$  & $\pm3.0$ \\
  Residual shape function & $\pm4.5$ \\
  Third order terms in the OPE  & $\pm4.0$ \\\hline\hline
  Total &  $\pm9.1$ \\ \hline\hline
\end{tabular}  
\end{small}
\end{center}
\label{tab:bulnuBLLerror}
\end{table}

\begin{figure}
\begin{center}
\includegraphics[width=6.0in]{figures/slb/vub_allMoments_BLL.eps}
\end{center}
\caption{Measurements of $\vub$ from inclusive semileptonic decays 
and their average in the BLL prescription.
``$(M_X, q^2)$'' indicates the analysis type.}
\label{fig:BLL}
\end{figure}


==> tables/slb/BLNP.tex <==
\begin{table}[!htb]
\caption{Summary of inclusive determinations with the investigated acceptance 
region in the analysis and their determination of $\vub$ in the BLNP prescription 
together with their average. The errors quoted on \vub\ correspond to
experimental and theoretical uncertainties, respectively.  The
$s_\mathrm{h}^{\mathrm{max}}$ variable is described in Ref.~\cite{ref:shmax}. }
\begin{center}
\begin{small}
\begin{tabular}{|llcc|}
\hline
%& $N_{B\Bb}\time 10^6$ & ${\Delta\mathcal{B}}(\bulnu) [10^{-4}] $
& accepted region & $f_u$
&  $\Vub [10^{-3}]$\\
\hline\hline
CLEO~\cite{ref:cleo-endpoint}
& $E_e>2.1\,\gev$ & 0.13
& $4.09\pm 0.48\pm 0.37$ \\ 
BELLE~\cite{ref:belle-endpoint}
& $E_e>1.9\,\gev$  & 0.24
& $4.82\pm 0.45\pm 0.30$ \\ 
\babar~\cite{ref:babar-endpoint}
& $E_e>2.0\,\gev$  & 0.19
& $4.39\pm 0.25\pm 0.32$ \\ 
\babar~\cite{ref:babar-elq2}
& $E_e>2.0\,\gev$, $s_\mathrm{h}^{\mathrm{max}}<3.5\,\mathrm{GeV^2}$ & 0.13
& $4.57\pm 0.31\pm 0.42$ \\
BELLE~\cite{ref:belle-mx}
& $M_X<1.7\,\gev/c^2$   & 0.47
& $4.06 \pm 0.27 \pm 0.24$ \\
BELLE~\cite{ref:belle-mxq2Anneal}
& $M_X<1.7\,\gev/c^2, q^2>8\,\gev^2/c^2$ & 0.24
& $4.37 \pm 0.46 \pm 0.29$ \\ 
\babar~\cite{ref:babar-q2mx}
& $M_X<1.7\,\gev/c^2, q^2>8\,\gev^2/c^2$ & 0.24
& $4.75 \pm 0.35 \pm 0.31$ \\ 
\hline\hline
{\bf Average}
& \mathversion{bold}$\chi^2=6/6$, CL$=0.41$ &
& \mathversion{bold}$4.52 \pm 0.19 \pm 0.27$ \\
\hline
\end{tabular}\\
\end{small}
\end{center}
\label{tab:bulnuBLNP}
\end{table}

\begin{table}[!htb]
\caption{Summary of uncertainties on the $\vub$ average in the BLNP prescription.}
\begin{center}
\begin{small}
\begin{tabular}{|lr|} \hline
  Source & Uncertainty(\%) \\ \hline \hline
  Statistics & $\pm2.1$ \\
  Detector & $\pm2.7$ \\
  $B\to X_c l \nu$ model & $\pm2.1$ \\
  $B\to X_u l \nu$ model & $\pm1.4$ \\
  Heavy quark parameters $m_b$ & $\pm4.1$ \\
  Sub-leading shape functions & $\pm0.9$ \\
  BLNP theory : Matching scales $\mu,\mu_i,\mu_h$  & $\pm3.8$ \\
  Weak annihilation  & $\pm2.1$ \\\hline\hline
  Total &  $\pm7.4$ \\ \hline
\end{tabular}  
\end{small}
\end{center}
\label{tab:bulnuBLNPerror}
\end{table}


==> tables/slb/DGE.tex <==

\begin{table}[!htb]
\caption{Summary of uncertainties on the $\vub$ average in the DGE prescription.}
\begin{center}
\begin{small}
\begin{tabular}{|lr|} \hline
  Source & Uncertainty(\%) \\\hline \hline
  Statistics & $\pm1.8$ \\
  Detector & $\pm2.5$ \\
  $B\to X_c l \nu$ model & $\pm2.3$ \\
  $B\to X_u l \nu$ model & $\pm2.3$ \\
  Spectral fraction ($m_b$) & $\pm1.2$ \\
  Strong coupling $\alpha_s$  & $\pm1.0$ \\
  Total semileptonic width ($m_b$)  & $\pm3.0$ \\
  DGE theory : matching scales   & $\pm2.9$ \\\hline\hline
  Total &  $\pm6.3$ \\ \hline
\end{tabular}  
\end{small}
\end{center}
\label{tab:bulnuDGEerror}
\end{table}

\begin{figure}
\begin{center}
\includegraphics[width=6.0in]{figures/slb/vub_allMoments_DGE.eps}
\end{center}
\caption{Measurements of $\vub$ from inclusive semileptonic decays 
and their average in the DGE description. 
``$E_e$'', ``$M_X$'', ``$(M_X,q^2)$'' and ``($E_e,s^{max}_h$)'' indicate the 
analysis type.}
\label{fig:DGE}
\end{figure}


==> tables/slb/bulnuDGE.tex <==

\begin{table}[!htb]
\caption{Summary of inclusive determinations with the investigate acceptance 
region in the analysis and their determination of $\vub$ in the DGE prescription 
together with their average. The errors quoted on \vub\ correspond to
experimental and theoretical uncertainties, respectively.  The
$s_\mathrm{h}^{\mathrm{max}}$ variable is described in Ref.~\cite{ref:shmax}. }
\begin{center}
\begin{small}
\begin{tabular}{|llcc|}
\hline
& accepted region & $f_u$
&  $\Vub [10^{-3}]$\\
\hline\hline
CLEO~\cite{ref:cleo-endpoint}
& $E_e>2.1\,\gev$ & 0.22
& $3.85\pm 0.45\pm 0.22$ \\ 
BELLE~\cite{ref:belle-endpoint}
& $E_e>1.9\,\gev$  & 0.37
& $4.80\pm 0.45\pm 0.20$ \\ 
\babar~\cite{ref:babar-endpoint}
& $E_e>2.0\,\gev$  & 0.30
& $4.29\pm 0.29\pm 0.21$ \\ 
\babar~\cite{ref:babar-elq2}
& $E_e>2.0\,\gev$, $s_\mathrm{h}^{\mathrm{max}}<3.5\,\mathrm{GeV^2}$ & 0.21
& $4.42\pm 0.30\pm 0.24$ \\
BELLE~\cite{ref:belle-mx}
& $M_X<1.7\,\gev/c^2$   & 0.64
& $4.29 \pm 0.28 \pm 0.22$ \\
BELLE~\cite{ref:belle-mxq2Anneal}
& $M_X<1.7\,\gev/c^2, q^2>8\,\gev^2/c^2$ & 0.36
& $4.42 \pm 0.47 \pm 0.19$ \\ 
\babar~\cite{ref:babar-q2mx}
& $M_X<1.7\,\gev/c^2, q^2>8\,\gev^2/c^2$ & 0.36
& $4.80 \pm 0.35 \pm 0.21$ \\ 
\hline\hline
{\bf Average}
& \mathversion{bold}$\chi^2=10/6$, \mathversion{bold}CL$=0.12$ &
& \mathversion{bold}$4.46 \pm 0.20 \pm 0.20$ \\
\hline
\end{tabular}\\
\end{small}
\end{center}
\label{tab:bulnuDGE}
\end{table}


==> tables/slb/dlnu.tex <==
% ----------------------------------------------------------------------0
\begin{table}[!htb]
\caption{Average of the branching fraction $\cbf(\BzbDplnu)$ and individual
results. }
\begin{center}
\begin{tabular}{|l|c|c|}\hline
Experiment                                 &$\cbf(\BzbDplnu) [\%]$ (rescaled) &$\cbf(\BzbDplnu) [\%]$ (published) \\
\hline\hline 
ALEPH ~\hfill\cite{Buskulic:1996yq}        &$2.15 \pm0.18_{\rm stat} \pm0.37_{\rm syst}$  &$2.35 \pm0.18_{\rm stat} \pm0.44_{\rm syst}$ \\
CLEO  ~\hfill\cite{Bartelt:1998dq}         &$2.07 \pm0.13_{\rm stat} \pm0.16_{\rm syst}$  &$2.20 \pm0.13_{\rm stat} \pm0.18_{\rm syst}$ \\
\belle  ~\hfill\cite{Abe:2001yf}           &$2.13 \pm0.12_{\rm stat} \pm0.39_{\rm syst}$  &$2.13 \pm0.12_{\rm stat} \pm0.41_{\rm syst}$ \\
\hline 
{\bf Average}                              &\mathversion{bold}$2.09 \pm0.18$      &\mathversion{bold}$\chi^2/\dof = 0.04/2$ (CL=$98\%$)  \\
\hline 
\end{tabular}
\end{center}
\label{tab:dlnu}
\end{table}
% ----------------------------------------------------------------------



==> tables/slb/gfits.tex <==

\begin{table}[!htb]
\caption{{\it Global fit} results for the {\it pole}, ``1S'' and {\it
  kinetic} schemes.}
\begin{center}
\begin{tabular}{|l|l|}\hline
  Source (Scheme)& Measurements \\
%  $|V_{cb}|(10^{-3})$/ $m_b$ or $\bar{\Lambda}$ GeV/$c^2$)   \\ 
\hline\hline 
Battaglia {\it et al.} (Kinetic)~\cite{Battaglia:2002tm}
& $|V_{cb}|=(41.9\pm 0.7_{meas}\pm0.6_{fit}\pm0.4_{pert})\times 10^{-3}$ \\
& $m_b^{\rm{kin}}=4.59 \pm 0.08_{fit}\pm 0.01_{syst.}\,\rm{GeV}/c^2$ \\
\hline
Battaglia {\it et al.} (Pole)~\cite{Battaglia:2002tm}
& $|V_{cb}|=(41.3\pm 0.7_{meas}\pm0.7_{fit}\pm0.2_{nl}\pm0.9_{pert})\times 10^{-3}$ \\
& $\mathrm{\bar{\Lambda}}=0.40 \pm 0.10_{fit}\pm
0.02_{syst.}\,\rm{GeV}/c^2$ \\
\hline
CLEO (Pole)~\cite{Mahmood:2002tt}
& $|V_{cb}|=(40.8\pm 0.5_{\Gamma_{\rm{SL}}}\pm0.4_{\lambda_1,\mathrm{\bar{\Lambda}}}\pm0.9_{theory})\times 10^{-3}$ \\
& $\mathrm{\bar{\Lambda}}=0.39 \pm 0.03_{stat}\pm0.06_{syst.}\pm0.12_{theory}\,\rm{GeV}/c^2$ \\
(1S) & $m_b^{\rm{1S}}=4.82 \pm
0.07_{exp}\pm0.11_{theory}\,\rm{GeV}/c^2$ \\
\hline
\babar (Kinetic)~\cite{Aubert:2004aw}
& $|V_{cb}|=(41.4 \pm 0.4_{exp}\pm0.4_{HQE}\pm0.6_{theory})\times 10^{-3}$ \\
& $m_b^{\rm{kin}}=4.61 \pm 0.05_{exp}\pm0.04_{HQE}\pm0.02_{theory}\,\rm{GeV}/c^2$ \\\hline
Bauer {\it et al.} (1S)~\cite{Bauer:2004ve}
&  $|V_{cb}|=(41.4 \pm 0.6 \pm0.1_{\tau_B})\times 10^{-3}$ \\
&  $m_b^{\rm{1S}}=4.68 \pm 0.03\,\rm{GeV}/c^2$ \\\hline
Buchm\"uller \& Fl\"acher (Kinetic)~\cite{Buchmuller:2005zv}
& $|V_{cb}|=(41.96 \pm 0.23_{exp}\pm0.35_{HQE}\pm0.59_{\Gamma_{\rm{SL}}})\times 10^{-3}$ \\
& $m_b^{\rm{kin}}=4.59 \pm 0.025_{exp}\pm0.030_{HQE}\,\rm{GeV}/c^2$ \\\hline
Belle (Kinetic)~\cite{Urquijo:ICHEP06}
& $|V_{cb}|=(41.93 \pm 0.65_{fit}\pm0.48_{\alpha_s}\pm0.68_{theory})\times 10^{-3}$ \\
& $m_b^{\rm{kin}}=4.564 \pm 0.076\,\rm{GeV}/c^2$ \\\hline
Belle ($1S$)~\cite{Urquijo:ICHEP06}
& $|V_{cb}|=(41.5 \pm 0.5_{fit}\pm0.2_{\tau_B})\times 10^{-3}$ \\
& $m_b^{\rm{1S}}=4.73 \pm 0.05\,\rm{GeV}/c^2$ \\
\hline 
\end{tabular}
\end{center}
\label{tab:gfits}
\end{table}

